CoLeaF: A Contrastive-Collaborative Learning Framework for Weakly Supervised Audio-Visual Video Parsing

Weakly supervised audio-visual video parsing (AVVP) methods aim to detect audible-only, visible-only, and audible-visible events using only video-level labels. Existing approaches tackle this by leveraging unimodal and cross-modal contexts. However, we argue that while cross-modal learning is beneficial for detecting audible-visible events, in the weakly supervised scenario, it negatively impacts unaligned audible or visible events by introducing irrelevant modality information. In this paper, we propose CoLeaF, a novel learning framework that optimizes the integration of cross-modal context in the embedding space such that the network explicitly learns to combine cross-modal information for audible-visible events while filtering them out for unaligned events. Additionally, as videos often involve complex class relationships, modelling them improves performance. However, this introduces extra computational costs into the network. Our framework is designed to leverage cross-class relationships during training without incurring additional computations at inference. Furthermore, we propose new metrics to better evaluate a method's capabilities in performing AVVP. Our extensive experiments demonstrate that CoLeaF significantly improves the state-of-the-art results by an average of 1.9% and 2.4% F-score on the LLP and UnAV-100 datasets, respectively.

==> test.tex <==



\vspace{2mm}
\noindent{\bf Hybrid Attention Network (HAN) -- } HAN \cite{tian2020unified} is a popular baseline for the weakly supervised AVVP task. In HAN, first, two pre-trained models are applied on the audio and visual signals of the input video $S$ to extract segment-level audio and visual input tokens, $F^a=\{f^{a}_{t}\}^{T}_{t=1}$ and $F^v=\{f^{v}_{t}\}^{T}_{t=1}$, respectively. Then, it aggregates unimodal and cross-modal information through applying and combining self-attention and cross-attention mechanisms \cite{vaswani2017attention} on the input tokens 
\begin{equation}
{\hat{f}}^{a}_{t} = {f}^{a}_{t} + \text{Self-attn}({f}^{a}_{t}, {F}^{a}) + \text{Cross-attn}({f}^{a}_{t}, {F}^{v}),
\end{equation}\vspace{-4mm}
% \begin{equation}
% {\hat{f}}^{\phi}_{t} = {f}^{\phi}_{t} + \text{Self-attn}({f}^{\phi}_{t}, {F}^{\phi}) + \text{Cross-attn}({f}^{\phi}_{t}, {F}^{\phi^{\bullet}}),
% \end{equation}
\begin{equation}
{\hat{f}}^{v}_{t} = {f}^{v}_{t} + \text{Self-attn}({f}^{v}_{t}, {F}^{v}) + \text{Cross-attn}({f}^{v}_{t}, {F}^{a}),
\end{equation}
% where $\phi\in\{a,v\}$ and $\phi^{\bullet}$ indicates the complementary modality of $\phi$.
\noindent Finally, HAN uses a share fully connected layer FC to predict multi-class segment-level audio and visual event probabilities from the audio and visual output tokens as ${P}^{\phi} = Sigmoid(FC(\hat{F}^{\phi}))$, where $P^{\phi}=\{{p}^{\phi}_{t}\in \rm {I\!R}^{1\times C}\}^{T}_{t=1}$. During the inference $P^{\phi}$ is utilized to predict segment-level audible-only, visible-only, and audible-visible events. However, during the training, as we only have video-level labels, HAN applies a Multimodal Multiple Instance Learning (MMIL) module to provide video-level probabilities as 
% \fan{say how HAN works at the inference}
\begin{equation}
\small
\label{eq: pt1}
W^{\vartriangle} = \textit{Soft-max}_{t}(FC_{t}([\hat{F}^a;\hat{F}^v]), ~
W^{\blacktriangle} = \textit{Soft-max}_{av}(FC_{av}([\hat{F}^a;\hat{F}^v]), 
\end{equation}\vspace{-4mm}
% \begin{equation}
% {P} = [P^a; P^v],
% \end{equation}
\begin{equation}
\small
\label{eq: pt2}
\mathbb{P} = \sum_{t=1}^{T} \sum_{m=1}^{M} (W^{\vartriangle}_{t,m}\odot W^{\blacktriangle}_{t,m}\odot{P}_{t,m}), ~ \text{where } {P} = [P^a; P^v], 
\end{equation}
and $M\hspace{-0.4em}=\hspace{-0.4em}2$ refers to audio and visual modalities, ${P},W^{\vartriangle},W^{\blacktriangle}\in \rm {I\!R}^{T\times 2\times C}$, $\mathbb{P}\in \rm {I\!R}^{1\times C}$, and $[;]$ and $\odot$ indicates the concatenation and Hadamard product operations, respectively.  $\textit{Soft-max}_{t}$ and $\textit{Soft-max}_{av}$ represent the Softmax layers along the temporal and audio-visual dimensions, respectively. With the video-level probabilities $\mathbb{P}$, and the video-level labels $Y$, HAN is optimized through Binary Cross Entropy (BCE) loss $\mathcal{{L}}_{video} = BCE(Y, \mathbb{P})$. 

\begin{figure}[t]
  \centering
  \includegraphics[width=0.85\linewidth]{Figuers/2CoLeaF.png}
  \caption{Our proposed framework {\method} consists of two network branches, {\r} and {\a}. The {\r} branch focuses on unimodal and their cross-class relationships, while the {\a} branch exploits both unimodal and cross-modal contexts. They work collaboratively to optimize the integration of cross-modal information for the AVVP task, leveraging only the video-level labels for training.}
  % \caption{Our proposed contrastive-collaborative framework {\method} has two network branches, {\r} and {\a}, which are trained simultaneously using the same audio and visual input data to tackle the weakly supervised AVVP task. {\r} focuses on unimodal and their cross-class relationships, while {\a} exploits unimodal and cross modal contexts. The branches are trained through the conventional video-level losses, $\mathcal{{L}}^{Ref}_{video}$ and $\mathcal{{L}}^{Anch}_{video}$, and our proposed collaborative losses $\mathcal{{L}}^{Ref}_{MoSelf}$, $\mathcal{{L}}^{Anch}_{MoEvt}$, and $\mathcal{{L}}^{Anch}_{CoCls}$. In inference, {\a} is deployed for the AVVP task.}
  \label{fig:2CoLeaF}
  \vspace{-3mm}
\end{figure}

\subsection{{\method}: Contrastive-Collaborative Learning Framework}
In this section, we introduce our proposed approach  {\method}, a novel collaborating learning framework, designed to address two key challenges in the weakly supervised AVVP task: (i) effectively integrating cross-modal contexts with the lack of modality-specific annotations, and (ii) efficiently learning cross-class relationships. {\method} comprises two network branches, {\r} and {\a}, as shown in Fig. \ref{fig:2CoLeaF}. The {\r} branch, used only during training, focuses on mining unimodal and co-occurrence class relationships. The {\a} branch exploits and combines unimodal and cross-modal contexts serving as the main network branch that is deployed during inference. Both network branches process the same audio and visual input data and are trained simultaneously using two types of losses: (a) the conventional video-level weakly supervised loss, as in HAN, and (b) {our proposed contrastive and distillation losses}. In the following, we explain the details of each branch and the losses.
% In this section, we introduce our novel learning framework, {\method}, designed to address two key challenges in the weakly supervised AVVP task: (i) effectively integrating cross-modal contexts with the lack of modality-specific annotations, and (ii) efficiently learning cross-class relationships. {\method} comprises two network branches, {\r} and {\a}, as shown in Fig. \ref{fig:2CoLeaF}. The {\r} branch, used only during training, focuses on mining unimodal and co-occurrence class relationships. The {\a} branch exploits and combines unimodal and cross-modal contexts serving as the main network branch that is deployed during inference. Both network branches process the same audio and visual input data and are trained simultaneously using two types of losses: (a) the conventional video-level weakly supervised loss, as in HAN, and (b) our proposed losses designed to tackle the two challenges we mentioned. In the following, we explain the details of each branch and the losses.

% \vspace{1mm}
\noindent{\bf {\r} Branch -- } This branch addresses weakly supervised AVVP by primarily focusing on unimodal information. This can be achieved by applying two self-attention layers on the audio and visual input tokens individually. However, as videos with multi-label events contain complex relationships between the event classes, we simultaneously leverage these information to improve the method’s performance. To model explicitly the cross-class relationships, inspired by \cite{mo2022multi}, we first concatenate the audio and visual input tokens, $F^{a}\hspace{-0.3em}=\hspace{-0.3em}\{f^{a}_t\}^{T}_{t=1}$ and $F^{v}\hspace{-0.3em}=\hspace{-0.3em}\{f^{v}_t\}^{T}_{t=1}$, with learnable audio and visual class tokens, $C^{a}\hspace{-0.3em}=\hspace{-0.3em}\{c^{a}_i\}^{C}_{i=1}$ and $C^{v}\hspace{-0.3em}=\hspace{-0.3em}\{c^{v}_i\}^{C}_{i=1}$. We then forward them into our self-attention backbones to exploit both intra-modality and class relationships,
\begin{gather}
\small
    {X}^{\phi}=\{{x}^{\phi}_{n}\}^{T + C}_{n=1}=[\{f^{\phi}_t\}^{T}_{t=1};\{c^{\phi}_i\}^{C}_{i=1}],\\
    \{\ddot{x}^{\phi}\}^{T+C}_{n=1}= \{\text{Self-attn}_{\phi}({x}^{\phi}_{n}, {X}^{\phi})\}^{T + C}_{n=1},
\end{gather}
% \begin{equation}
% \small
%     {X}^{\phi}=\{{x}^{\phi}_{n}\}^{T + C}_{n=1}=[\{f^{\phi}_t\}^{T}_{t=1};\{c^{\phi}_i\}^{C}_{i=1}],
% \end{equation}\vspace{-2mm}
% \begin{equation}
% \small
% \{\ddot{x}^{\phi}\}^{T+C}_{n=1}= \{\text{Self-attn}_{\phi}({x}^{\phi}_{n}, {X}^{\phi})\}^{T + C}_{n=1},
% \end{equation}
where $\phi\in\{a,v\}$ and $[;]$ indicates the concatenation operations. We take the output of self-attention layers which are correspond to the audio and visual input tokens, $\ddot{F}^{\phi}=\{\ddot{x}^{\phi}_n\}^T_{n=1}$, to predict segment-level audio and visual event probabilities through a fully connected layer as $\{\ddot{p}^{\phi}_{t}\}^T_{t=1} = Sigmoid(FC_{\phi}(\ddot{F}^{\phi}))$, where $\ddot{p}^{\phi}_{t}\in \rm {I\!R}^{1\times C}$. Subsequently, the audio and visual event probabilities are computed as ${\ddot{\mathcal{P}}}^{\phi} =\sum_{t=1}^{T}(\ddot{w}^{\phi}_{t}\odot \ddot{p}^{\phi}_{t})$,
% \begin{equation}
% \small
%     {\ddot{\mathcal{P}}}^{\phi} =\sum_{t=1}^{T}(\ddot{w}^{\phi}_{t}\odot \ddot{p}^{\phi}_{t}),
% \end{equation}
where ${\ddot{\mathcal{P}}}^{\phi},\ddot{w}_{t}\in \rm {I\!R}^{1\times C}$, and $\ddot{w}_{t}$ are temporal learnable weight. With the audio and visual  event probabilities and video-level annotations $Y\in \rm {I\!R}^{1\times C}$, the {\r} branch is optimized through the video-level loss $\mathcal{{L}}^{Ref}_{video} = \sum_{\phi\in\{a,v\}}BCE(Y, \ddot{\mathcal{P}}^{\phi})$.
% , where $\ddot{P}^{\phi}=\{\ddot{p}^{\phi}\}^{T}_{t=1}$.


Optimizing the {\r} branch by relying only on the $\ddot{F}^{\phi}$ output tokens does not guarantee that the input class tokens learn to model the class events. To ensure that they represent the classes effectively, we also utilize the output tokens of self-attention layers which are correspond to the input class tokens, $\{\ddot{c}^{\phi}\}^{C}_{i=1}=\{\ddot{x}^{\phi}_n\}^{T+C}_{n=T+1}$, for the network optimization. To achieve this, we apply a global average pooling layer on these tokens along their embedding dimension to convert them into a 1-D dimensional vector, followed by a sigmoid activation function to convert them into range 0 and 1 as $CLS^{\phi}=\{ Sigmoid(AvgPool(\ddot{c}^{\phi}_i))\}^{C}_{i=1}$. Then they are supervised by video-level annotations and cross entropy loss. Therefore, the video-level loss is extended as $\mathcal{{L}}^{Ref}_{video} = \sum_{\phi\in\{a,v\}}\hspace{-0.3em}BCE(Y, \ddot{\mathcal{P}}^{\phi}) + BCE(Y, {CLS}^{\phi})$.

\noindent{\bf {\a} Branch -- } This  branch addresses the weakly supervised AVVP task by exploiting both unimodal and cross-modal contexts. To achieve this, a backbone that performs the AVVP task using self-attention and cross-attention mechanisms (\eg, HAN) can serve as {\a} to predict segment-level and video-level probabilities $P^{\phi}=\{p^{\phi}_t\in \rm {I\!R}^{1\times C}\}^T_{t=1}$ and $\mathbb{P}\in \rm {I\!R}^{1\times C}$ (Eqs \ref{eq: pt1}-\ref{eq: pt2}), respectively, from the audio and visual input tokens $F^{\phi}$. The segment-level labels are employed for inference phase, as well as later in this section for {our proposed self-modality-aware knowledge distillation loss}, while the video-level probabilities are utilized to compute the video-level loss $\mathcal{{L}}^{Anch}_{video}=BCE(Y,\mathbb{P})$, as in HAN network.

% \vspace{1.0mm}
\noindent {\bf Event-Aware Contrastive Learning -- } Although leveraging cross-modal information is beneficial for the detection of audible-visible events, we argue that in the weakly supervised scenario, it can negatively impact the detection of unaligned audio-visible events by introducing irrelevant modality information. This argument is supported by our findings in Table \ref{tab:different modality}. To tackle this challenge, we introduce contrastive learning to explicitly optimize the integration of unimodal and cross-modal contexts in audio and visual output tokens of the {\a} branch ${\hat{f}}^{\phi}_{t}$. To do this, the output tokens of the corresponding segment from the {\r} branch $\ddot{x}^{\phi}_t$ can be chosen as a positive sample, and the output tokens of the rest of its segments can be considered as negative set. Subsequently, the {\a} branch can be optimized through Noise Contrastive Estimation (NCE) loss \cite{gutmann2010noise}.  In this formulation, regardless of the event types in a video, {\a} is encouraged to learn similar representations with {\r}. However, in the AVVP task, the video can contain multiple events, diversely spanning audible-only, visible-only, and audible-visible, and our goal is to get close to the tokens' representations of the {\r} branch for only unaligned audio-visible event types. We address this issue by introducing a novel event-aware NCE loss that adapts the strength of contrastive learning encouragement based on the degree of audible-only and visible-only events present in the input video 

\begin{equation}
\small
    \mathcal{L}^{Anch}_{Evt} = - \frac{1}{T} * \sum_{\phi\in\{a,v\}}\vartheta^{\phi} *\sum_{t=1}^{T}\log{\frac{\exp{({{\hat{f}^{\phi}}_{t}}^{\intercal}.{\ddot{x}^{\phi}}_{t}/\tau)}}{\sum_{n=1,n\neq t}^{T}\exp{({{\hat{f}^{\phi}}_{n}}^{\intercal}.{\ddot{x}^{\phi}}_{n}/\tau)}}},
    % \log{\frac{\exp{({\hat{f}^{\phi}_{t}}^{T}.\ddot{x}^{\phi}_{t}/\tau)}}{\sum_{n}\exp{({\hat{f}^{\phi}_{n}}^{T}.\ddot{x}^{\phi}_{n}/\tau)}}
\end{equation}

\noindent where weight $\vartheta^{\phi}$ is computed from a set of pseudo-labels $\ddot{G}^{\phi}=\{\ddot{g}^{\phi}_i\}^C_{i=1}$ distilled from the {\r} branch 
\begin{gather}
    \small
    \ddot{g}^{\phi}_i = \begin{cases}
                           1 & \text{if $\ddot{\mathcal{P}}^{\phi}_i > \theta$}\\                                           0 & \text{else}
             \end{cases},\\
    N_{a} = \sum_{c=1}^{C} \ddot{g}^{a}_i \odot (1-\ddot{g}^{v}_i), N_{v} = \sum_{c=1}^{C} \ddot{g}^{v}_i \odot (1-\ddot{g}^{a}_i), N_{av} = \sum_{c=1}^{C} \ddot{g}^{a}_i \odot \ddot{g}^{v}_i,\\
    \vartheta^{a} = \frac{N_a}{N_a + N_{av}}, \text{   and    } \vartheta^{v} = \frac{N_v}{N_v + N_{av}}.
\end{gather}
% \begin{equation}
% \small
% \ddot{g}^{\phi}_i = \begin{cases}
%                            1 & \text{if $\ddot{\mathcal{P}}^{\phi}_i > \theta$}\\                                           0 & \text{else}
%              \end{cases},
% \end{equation}
% \begin{equation}
% \small
%     N_{a} = \sum_{c=1}^{C} \ddot{g}^{a}_i \odot (1-\ddot{g}^{v}_i), N_{v} = \sum_{c=1}^{C} \ddot{g}^{v}_i \odot (1-\ddot{g}^{a}_i), N_{av} = \sum_{c=1}^{C} \ddot{g}^{a}_i \odot \ddot{g}^{v}_i,
% \end{equation}
% \begin{equation}
% \small
%     \vartheta^{a} = \frac{N_a}{N_a + N_{av}}, \text{   and    } \vartheta^{v} = \frac{N_v}{N_v + N_{av}}
% \end{equation}
$N_a$, $N_v$, and $N_{av}$ indicate the number of audible-only, visible-only, and audible-visible events in the video, respectively. $\vartheta^{\phi}$ reflects the degree of encouragement in the contrastive learning and takes a value between 0 and 1 where 0 indicates there is no event or all the events are audible-visible, resulting in no encouragement, and 1 indicates all the events are unaligned, resulting in maximum encouragement.

\vspace{1.0mm}
\noindent {\bf Self-Modality-Aware Knowledge Distillation -- }
If the {\r} branch relies solely on {`modality-agnostic'} video-level labels for training, it faces two key limitations: (i) it cannot acquire rich representations necessary to teach {\a}, and (ii) our proposed event-aware contrastive loss may not effectively optimize cross-modal learning since it relies on the predicted event types. To overcome these, we propose to leverage free modality-aware knowledge from the {\a} branch to improve the performance of the {\r} branch. To perform this, we first distil pseudo labels ${G}^{\phi}=\{{g}^{\phi}_i\}^C_{i=1}$ from the estimated audio and visual event probabilities in the {\a} branch,
\begin{equation}
{g}^{\phi}_i = \begin{cases}
                           1 & \text{if ${\mathcal{P}}^{\phi}_i > \theta$}\\                                           0 & \text{else}
             \end{cases}
\end{equation} 
Then, ${G}^{\phi}$ are used to compute our proposed {self-modality-aware knowledge distillation loss} for the {\r} branch as $\mathcal{{L}}^{Ref}_{SelfMo}=\sum_{\phi\in\{a,v\}}BCE({G}^{\phi}, \mathcal{\ddot{P}}^{\phi})$.





\vspace{1.0mm}
\noindent{\bf{Co-occurrence Class Knowledge Distillation -- }} The primary goal of modeling the co-occurrence class relationships explicitly in the {\r} branch is to transfer them to the {\a} branch so that we can benefit from this knowledge during inference without suffering from the associated computation overhead. Optimizing the {\a} branch through our proposed contrastive learning may implicitly transfer class relationships from the {\r} branch to the {\a} branch, but cannot fully transfer them because it is not desgined for this purpose. To explicitly transfer the cross-class relationships, we introduce the co-occurrence class knowledge distillation loss, where we first obtain the audio and visual class correlation matrices, ${\ddot{M}^{\phi}}\in \rm{I\!R}^{C\times C}$ and ${{M}^{\phi}}\in \rm{I\!R}^{C\times C}$, for the {\r} and {\a} branches as 
\begin{equation}
\small
{\ddot{M}^{\phi}}_{i, j} = \ddot{\mathcal{P}}^{\phi}_{i}*\ddot{\mathcal{P}}^{\phi}_{j} \text{, and }{{M}^{\phi}}_{i,j} = {\mathcal{P}}^{\phi}_{i}*{\mathcal{P}}^{\phi}_{j}.
\end{equation}
By computing the correlations, we quantify the relationships between each pair of classes. Then, we encourage the {\a} branch to mimic the audio and visual cross-class correlations of the {\r} branch through the mean square error (MSE) as 
$\mathcal{{L}}^{Anch}_{CoCls} = \sum_{\phi\in\{a,v\}}MSE(\ddot{M}^{\phi},{M}^{\phi})$.

% \vspace{2mm}
% \fsn{\noindent \emph{Remark}: To the best of our knowledge, that is the first time the knowledge distillation is explored not only for tackling the AVVP task, but also for facilitating cross-modal learning and efficiently modeling cross-class relationships. }

\section{New Metrics for AVVP}
\label{sec: metrics}
Current approaches utilize 5 metrics, under segment-level and event-level, to evaluate the method's performance for the AVVP task. These metrics include F-score for audible-only (A), visible-only (V), and audible-visible (AV) events separately, as well as the average F-score of the A, V, and AV (Type@AV), and the overall F-score for all A and V events within each sample (Event@AV). To compute these metrics, they first employ a threshold on the estimated audio and visual event probabilities to identify audible and visible events, $\hat{y}^a_t$ and $\hat{y}^v_t$, respectively. Then, the F-score for A and V are computed by comparing $\hat{y}^a_t$ and $\hat{y}^v_t$ with their corresponding audio and visual ground-truth labels, ${y}^a_t$ and ${y}^v_t$, respectively. The F-score for AV instead is computed by simultaneously considering both audible and visible events and their ground-truth labels.

\noindent We argue that the A and V metrics fail to accurately evaluate the method's performance in detecting audible-only and visible-only events because they consider only their corresponding modalities. In contrast, we believe that both modalities should be considered when computing A and V, similar to AV.  For instance, consider a scenario where the network predicts $\hat{y}^{a}_{t}=1$ and $\hat{y}^{v}_{t}=1$ for an audible-only event with ground-truth labels $y^{a}_{t}=1$ and $y^{v}_{t}=0$. According to the A metric, this prediction is considered a true positive. However, when both modalities are considered, it becomes evident that the network's prediction is incorrect, as it predicted an audible-visible event instead of an audible-only event. Thus, this should be considered a false positive for the audible-only metric. Consequently, a network that excels at detecting audible-visible events may falsely exhibit high true positive rates for the A and V metrics. This issue becomes particularly prominent when using cross-modal context in a weakly supervised scenario, as methods under these settings inherently tend to detect events as audible-visible. To overcome this, we introduce `audible-only’ and `visible-only’ event proposals, $\hat{y}^{ao}_t$ and $\hat{y}^{vo}_t$, as well as `audible-only’ and `visible-only’ ground-truth labels, ${y}^{ao}_t$ and ${y}^{vo}_t$, that are derived by considering both modalities as 
\begin{equation}
    \hat{y}^{ao}_{t} = \hat{y}^{a}_{t} \odot (1 - \hat{y}^{v}_{t}),\text{ and } \hat{y}^{vo}_{t} = \hat{y}^{v}_{t} \odot (1 - \hat{y}^{a}_{t}),
\end{equation} \vspace{-6mm}
\begin{equation}
    {y}^{ao}_{t} = {y}^{a}_{t} \odot (1 - {y}^{v}_{t}),\text{ and }{y}^{vo}_{t,i} = {y}^{v}_{t} \odot (1 - {y}^{a}_{t}),
\end{equation}
These new event proposals and their corresponding ground-truth labels are used to compute the F-score for audible-only (Ao) and visible-only (Vo) events. Subsequently, we have Type@AVo, which computes the average F-score of Ao, Vo, and AV, and Event@AVo, which computes overall F-score for all Ao and Vo events within each sample.
 
\section{Experimental Results}
\noindent{\bf Dataset --} LLP \cite{tian2020unified} is the only benchmark dataset for the AVVP task. It comprises 11,849 10-second YouTube video clips spanning 25 event classes, offering a diverse range of video events. Notably, 7,202 of these videos contain multiple event categories. In the LLP dataset, videos are partitioned into training, validation, and testing sets. While the training set includes only video-level annotations, the validation and test sets feature annotations for individual audio and visual events with second-wise temporal boundaries.

\noindent{\bf Implementation Details --} 
 We implement the {\r} branch by employing two self-attention layers, \emph{i.e.}, one for each modality, followed by two fully connected layers that obtain the temporal weights and estimate class probabilities, respectively. For the {\a} branch, we employ CMPAE \cite{gao2023collecting} as the backbone. 
% By following the previous works 
Following previous works \cite{tian2020unified,gao2023collecting}, audio input tokens are extracted through pre-trained VGGish \cite{hershey2017cnn}, and visual tokens are obtained through the pre-trained models ResNet152 \cite{he2016deep} and R(2+1)D \cite{tran2018closer}. The feature dimension for all input tokens, including the class tokens, is set to 512, % consistent with
as in
previous approaches. To train {\method}, we utilized the Adam optimizer with an initial learning rate of $5 \times 10^{-4}$ and a batch size of 128 for 15 epochs. The learning rate was decayed by a factor of 0.25 every 6 epochs. Our experiments were performed using PyTorch on an NVIDIA GeForce RTX 3090 GPU.

\subsection{Ablation Studies}
\label{sec: ablations}
In this section, we examine the impact of key components of {\method}, using the Ao, Vo, and AV metrics on LLP.


\noindent{\bf Impact of Event-Aware Contrastive Learning -- } In this section, we evaluate the effect of our proposed contrastive loss, $\mathcal{L}^{Anch}_{Evt}$. We compare the performance of our framework against three variants: one without $\mathcal{L}^{Anch}_{Evt}$, and two where it is replaced with the standard NCE loss $\mathcal{L}_{NCE}$ and BCE loss $\mathcal{L}_{BCE}$, the latter using the pseudo-labels employed by $\mathcal{L}^{Anch}_{Evt}$. Table \ref{tab: contrastive loss} demonstrates that standard contrastive learning is ineffective for the AVVP task. While $\mathcal{L}_{BCE}$ yields average improvement, its effectiveness is not consistent across all event types, i.e., it deteriorates performance in detecting the visible-only events in both segment and event levels. Our contrastive loss tailored for this task increases the method’s performance across all event types (see blue numbers in Table~\ref{tab: contrastive loss}). Specifically, it leads to a significant improvement {({\bf{over 2\%}} F-score)} in detecting audible-only events in both segment and event levels.

% \vspace*{-3.4mm}
\noindent{\bf Impact of Self-Modality-Aware Knowldge -- } In Table~\ref{tab: self-loss}, we ablate our proposed loss $\mathcal{L}^{Anch}_{SelfMo}$. The results demonstrate that the additional modality-aware knowledge obtained by {\a} for {\r} during training eventually enhances the performance of {\a} itself across all event types, specifically resulting in {\bf over a 1\%} improvement in F-score for detecting unaligned audible-visible event types.
% In Table~\ref{tab: self-loss}, we ablate our proposed self-modality aware knowldge distilation loss $\mathcal{L}^{Anch}_{SelfMo}$. The results demonstrate that leveraging the modality-aware knowledge obtained from the {\r} branch leads to its improvements across all event types, specifically resulting in over a 1\% F-score improvement for audio-visible unaligned event types.

% \vspace*{-20mm}
\noindent{\bf Impact of Learning Co-occurrence Class Relationships -- } In {\method}, the class tokens and $\mathcal{{L}}^{Anch}_{CoCls}$ are introduced to explicitly model the cross-class relationships in {\r} and facilitate their transfer to {\a}. In Table~\ref{tab: class relationships}, we ablate these two components. The results show that the network can benefit from $\mathcal{{L}}^{Anch}_{CoCls}$ with and without using the class tokens as it improves the method’s performance in both scenarios. However, the most improvement on average is achieved when it is used with the class tokens, \ie, {\bf{over a 1\%}} F-score improvement on all event types in comparison with when none of them are employed (see blue numbers in Table~\ref{tab: class relationships}). In these experiments, we also observed that using the class tokens increased the computational complexity of {\r} by 41.7\% Flops (\ie, from 12.7 to 18.0 GFlops) for 25 classes of LLP. However, our novel design in {\method} allows us to benefit from the knowledge learned from the class tokens without suffering from their computational overhead in the inference. Notably, this novel design can benefit other video understanding tasks where exploiting class dependencies is crucial.


\noindent{\bf Framework Generalization --} {\method} is a general learning framework, which means that any existing AVVP method can be embedded in our framework to (i) explicitly optimize the integration of cross-modal information and (ii) benefit from modeling co-occurrence class relationships in an end-to-end manner. In Table \ref{tab: framework generalization}, we present two examples: HAN \cite{tian2020unified}, a common architecture for AVVP, and CMPAE \cite{gao2023collecting}. The results demonstrate that our proposed framework significantly enhances the performance of HAN and CMPAE, \ie, on average, their F-score is increased by {\bf{2.4\%}}. This improvement is achieved in an end-to-end manner without requiring additional annotations or altering their network architecture.


% \noindent{\bf Contribution of Different Distillation Losses -- }
% In the {\method} framework, we introduced three different knowledge distillation losses: $\mathcal{L}^{Uni}$, $\mathcal{L}^{Cross}$, and $\mathcal{L}^{Co}$. Table \ref{tab: mimicry losses} evaluates the performance of {\method} by removing each of these losses. The results reveal that while the co-occurrence class distillation loss $\mathcal{L}^{Co}$ contributes to the detection of all event types, the unimodal and cross-modal distillation losses, $\mathcal{L}^{Uni}$ and $\mathcal{L}^{Cross}$, primarily enhance the method's performance (\emph{\ie}, {\a}'s performance) in detecting audible-only and visible-only events, in line with their design purpose. $\mathcal{L}^{Co}$ highly increases the AV F-score by {\bf 1.4\%} on both segment-level and event-level, and $\mathcal{L}^{Uni}$ leads to a significant improvement in visible-only Vo F-score by {\bf 2.9\%} and {\bf 2.6\%} at the segment and event levels, respectively. 

\begin{table}[t]
\scalebox{0.8}
{
  \floatsetup{captionskip=4pt}
  \begin{floatrow}[2]
    \hspace{-20mm}
        \ttabbox%
    {\setlength{\tabcolsep}{1 pt} % Default value: 6pt
    \renewcommand{\arraystretch}{0.95}
    \begin{tabularx}{0.572\textwidth}{@{}l ccc c ccc @{}}
      \specialrule{.2em}{.1em}{.1em}
     \multirow{2}{*}{Loss}& \multicolumn{3}{c}{Segment-level}&~\phantom & \multicolumn{3}{c}{Event-level}\cr \cmidrule{2-4} \cmidrule{6-8}
      & Ao& Vo& AV&\phantom& Ao& Vo& AV\cr \specialrule{.2em}{.1em}{.1em} 
    % \multicolumn{1}{c}{-} &  47.2& 61.8& 56.9& &41.2&61.7&50.5 \cr \cmidrule{2-8} 
     $\mathcal{L}_{NCE}$& 46.1& 60.8& 56.3& &40.5&60.6&50.1 \cr 
     $\mathcal{L}_{BCE}$& {48.5}& {61.2} & {57.4} & & {43.5}& {61.1}& {51.2}\cr \specialrule{.2em}{.1em}{.1em}
     \multicolumn{1}{c}{\bf-} &  47.3& 61.8& 56.7& &41.6&61.7&50.3 \cr\cmidrule{1-8}
     $\mathcal{L}^{Anch}_{Evt}$& {\bf49.3}& {\bf62.4}& {\bf58.6}& & {\bf44.1}& \bf{62.2}& {\bf52.1} \cr 
     & \blue{(+2.1)}& \blue{(+0.6)}& \blue{(+0.9)}& & \blue{(+2.5)}&\blue{(+0.5)}&\blue{(+0.8)}\cr \specialrule{.2em}{.1em}{.1em}
     % &  && \blue{(-1.5)}& \blue{(-1.1)}& \blue{(-1.8)}& & \blue{(-1.5)}&\blue{(-1.1)}&\blue{(-2.1)} \cr\cmidrule{1-10}
     % \cmark& &\cmark& {\bf49.5}&{\bf62.1}&{\bf58.6}& &{\bf44.2}&{\bf61.9}& {\bf52.0}\cr \specialrule{.2em}{.1em}{.1em}
      \end{tabularx}}
    {\caption{Ablation studies on $\mathcal{L}^{Anch}_{Evt}$.}
  \label{tab: contrastive loss}}
    \ttabbox%
    {
    \setlength{\tabcolsep}{2 pt} % Default value: 6pt
    \renewcommand{\arraystretch}{1.1}
    
    \begin{tabularx}{0.645\textwidth}{c ccc c ccc}
      \specialrule{.2em}{.1em}{.1em}
      \multirow{2}{*}{$\mathcal{{L}}^{Anch}_{SelfMo}$}& \multicolumn{3}{c}{Segment-level}&\phantom & \multicolumn{3}{c}{Event-level}\cr \cmidrule{2-4}  \cmidrule{6-8}
    &  \multicolumn{1}{c}{Ao}& \multicolumn{1}{c}{Vo}& \multicolumn{1}{c}{AV}&\phantom& \multicolumn{1}{c}{Ao}& \multicolumn{1}{c}{Vo}& \multicolumn{1}{c}{AV}\cr \specialrule{.2em}{.1em}{.1em}
     \xmark &  48.1& 60.9& 57.9& & 42.8&60.6&51.4\cr \cmidrule{1-8}
     % \xmark &\cmark &  47.2& 61.8& 56.9& &41.2&61.7&50.5 \cr\cmidrule{3-9}
     \cmark  & {\bf49.5}& {\bf62.1}& {\bf58.6}& & {\bf44.2}& {\bf61.9}& {\bf52.0}\cr 
     & \blue{(+1.4)}& \blue{(+1.2)}& \blue{(+0.7)}& & \blue{(+1.4)}&\blue{(+1.3)}&\blue{(+0.6)}\cr\specialrule{.2em}{.1em}{.1em}
      \end{tabularx}}
    {\caption{Ablation studies on $\mathcal{L}^{Ref}_{SelfMo}$.}
  \label{tab: self-loss}}
    % \hfill%
  \end{floatrow}}
\end{table}%

\begin{table}[t]
\scalebox{0.80}
{
  \floatsetup{captionskip=4pt}
  \begin{floatrow}[2]
    \hspace{-22mm}
        \ttabbox%
    {\setlength{\tabcolsep}{0.6 pt} % Default value: 6pt
    \renewcommand{\arraystretch}{0.99}
    \begin{tabularx}{0.64\textwidth}{@{}cc c ccccccc @{}}
      \specialrule{.2em}{.1em}{.1em}
      \multirow{2}{*}{Tkn}& ~~\phantom &\multirow{2}{*}{$\mathcal{{L}}^{Anch}_{CoCls}$} & \multicolumn{3}{c}{Segment-level}&~\phantom & \multicolumn{3}{c}{Event-level}\cr \cmidrule{4-6} \cmidrule{8-10}
      & & & Ao& Vo& AV&\phantom& Ao& Vo& AV\cr \specialrule{.2em}{.1em}{.1em}
      \cmark& & \xmark& 47.5& 60.3& 57.0& &41.9&60.2&50.4 \cr 
     \xmark& &\cmark& 48.2& {\bf62.7}& 57.3& &42.5&{\bf62.5}& 52.0\cr \specialrule{.2em}{.1em}{.1em}
     \xmark& &\xmark& 47.8& 60.8& 56.6& &42.2&60.6&49.8 \cr \cmidrule{1-10}
     \cmark& &\cmark& {\bf49.3}&{62.4}&{\bf58.6}& &{\bf44.1}&{62.2}& {\bf52.1}\cr &  && \blue{(+1.1)}& \blue{(+1.6)}& \blue{(+2.0)}& & \blue{(+1.9)}&\blue{(+1.6)}&\blue{(+2.3)} \cr\specialrule{.2em}{.1em}{.1em}
      \end{tabularx}}
    {\caption{Ablation studies on class tokens (Tkn) and $\mathcal{{L}}^{Anch}_{CoCls}$.}
  \label{tab: class relationships}}
    \ttabbox%
    {
    \setlength{\tabcolsep}{0.8 pt} % Default value: 6pt
    \renewcommand{\arraystretch}{0.8}
    
    \begin{tabularx}{0.635\textwidth}{lccccccc}
      \specialrule{.2em}{.1em}{.1em}
      &\multicolumn{3}{c}{Segment-level}&&\multicolumn{3}{c}{Event-level}\cr \cmidrule{2-4} \cmidrule{6-8}
      & Ao& Vo& AV&~\phantom& Ao& Vo& AV\cr \specialrule{.2em}{.1em}{.1em}
      HAN \cite{tian2018audio}& 33.1& 50.7& 48.9& & 31.0&50.1&43.0 \cr \cmidrule{1-8}
     HAN$\circledast$ & {\bf36.3}& {\bf54.1}& {\bf49.4}& & {\bf34.2}& {\bf53.5}& {\bf43.7}\cr
     & \blue{(+3.2)}& \blue{(+3.4)}& \blue{(+0.5)}& & \blue{(+3.2)}& \blue{(+3.4)}& \blue{(+0.7)}\cr \specialrule{.2em}{.1em}{.1em}
    CMPAE \cite{gao2023collecting}& 48.2& 57.9& 57.5& & 43.6&57.5&49.6 \cr \cmidrule{1-8}
            CMPAE$\circledast$& {\bf49.3}& {\bf62.4}& {\bf58.6}& & {\bf44.1}& {\bf62.1}& {\bf52.1}\cr 
    & \blue{(+1.1)}& \blue{(+4.5)}& \blue{(+1.1)}& & \blue{(+0.5)}& \blue{(+4.6)}& \blue{(+2.5)}\cr \specialrule{.2em}{.1em}{.1em}
      \end{tabularx}}
    {\caption{Framework generalization on LLP. $\circledast$ indicates that the network has been embedded in {\method} as the {\a} branch.}
  \label{tab: framework generalization}}
    % \hfill%
  \end{floatrow}}
\end{table}%

\subsection{State-of-the-Art Comparison} 
In this section, we compare the performance of {\method} with current state-of-the-art approaches using both traditional and our proposed metrics. The results of the previous methods under the new metrics were reproduced using their available code whenever accessible. Note that to obtain the event proposals from the estimated output probabilities, CMPAE \cite{gao2023collecting} utilizes a set of `selected thresholds’ for different event categories of LLP, while in the standard setting used by other state-of-the-art approaches, a fixed threshold is applied to all event classes. For a fair comparison, we also present the CMPAE’s results under the standard setting.

\begin{table}[t]

\caption{Weakly supervised AVVP results on the LLP dataset when utilizing video-level labels for training. All methods use VGGish, ResNet152, and R(2+1)D to generate the input tokens. `T@' and `E@' refers `Type@AV' and `Event@AV', respectively. {$\dag$} indicates the results are under {`selected thresholds'} setting. The best and the second-best results are in {\bf Bold} and \underline{underlined}, respectively.\vspace{-3mm}}
  \label{tab: SOTA-weak}
\centering
\scalebox{0.75}
{ \hspace{-7.8mm}
  \setlength{\tabcolsep}{0.1pt} % Default value: 6pt
    \renewcommand{\arraystretch}{0.85} % Default value: 1
  \begin{tabular}{@{}l c ccccccccc c ccccccccc @{}}\specialrule{.2em}{.1em}{.1em}
    \multirow{2}{*}{Method}&\phantom & \multicolumn{9}{c}{Segment-level (\%)}&\phantom & \multicolumn{9}{c}{Event-level (\%)}\cr \cmidrule{3-11} \cmidrule{13-21}
    & \phantom & A&Ao& V&Vo& AV& T@&T@o & E@&E@o&\phantom& A&Ao& V&Vo& AV& T@&T@o & E@&E@o\cr \specialrule{.2em}{.1em}{.1em}
    AVE \cite{tian2018audio}&  & 47.2&--& 37.1&--& 35.4& 39.9&~~--~ &41.6&--&~~& 40.4&--& 34.7&--&31.6&35.5&~~--~& 36.5&--\cr
    AVSDN \cite{lin2019dual} & & 47.8&--&52.0&-- & 37.1& 45.7&--& 50.8&--&~~& 34.1&--& 46.3&--& 26.5&35.6&--& 37.7&--\cr
    CVCMS \cite{lin2021exploring}& & 59.2&--& 59.9&--& 53.4& 57.5&--& 58.1&--&~~& 51.3&--& 55.5&--& 46.2& 51.0&--& 49.7&-- \cr
    
    MM-Pyr \cite{yu2022mm} & & 60.9&--& 54.4&--& 50.0& 55.1&--&57.6&--& & 52.7&--& 51.8&--& 44.4& 49.9&--& 50.5&--\cr
    DHHN \cite{jiang2022dhhn} & & 61.3&--& 58.3&--& 52.9& 57.5&--&58.1&--& & 54.0&--&55.1&-- & 47.3& 51.5&--& 51.5&--\cr
    MGN \cite{mo2022multi} & & 60.8&--& 55.4&--& 50.0& 55.5&--&57.2&--& & 51.1&--& 52.4&--& 44.4& 49.3&--& 49.1&--\cr \cmidrule{3-21}
    HAN \cite{tian2020unified}& &{60.1}&33.1&52.9&50.7&48.9&54.0&44.3&55.4&24.1& &51.3&31.0&48.9&50.1&43.0&47.7&41.4&48.0&22.0\cr
    MA \cite{wu2021exploring}& & {60.3}&43.5& 60.0&53.6& 55.1& 58.9&50.8&57.9&32.0& & 53.6&38.8& 56.4&52.4& 49.0& 53.0&46.8& 50.6&27.8\cr
    JoMoLD \cite{cheng2022joint}& & {61.3}&46.2&\underline{63.8}&\underline{58.8} &{57.2} &60.8&\underline{54.4} &59.9&35.4 &~~& 53.9&40.9&59.9&\underline{59.0} &\underline{49.6} & 54.5&\underline{50.3}& 52.5&31.1\cr
    CMPAE \cite{gao2023collecting}& &\bf{{63.9}}&\underline{48.2} & 63.3&57.9& \underline{57.5}& \underline{61.2}&54.2&\bf{62.1}&\underline{35.7}& & \bf{57.1}&\underline{43.6}& \underline{60.6}&57.5& \underline{49.6}& \underline{55.8}&\underline{50.3}& \underline{55.6}&\underline{32.0}\cr \cmidrule{1-21} 
    {{\method}} & & {\underline{63.5}}&{\bf49.3}& {\bf64.5}&{\bf62.4}& {\bf58.6}& {\bf62.1}&{\bf56.7}&\underline{61.8}&{\bf37.7}& & \underline{56.2}&{\bf44.1}& {\bf62.0}&{\bf62.2}& {\bf52.1}&{\bf56.7}&{\bf52.7} & {\bf54.5}&{\bf33.4}\cr 
    & & &\blue{(+1.1)}& &\blue{(+3.6)}& \blue{(+1.1)}& &\blue{(+1.4)}&~~&\blue{(+2.0)}& & &\blue{(+0.5)}& &\blue{(+2.2)}& \blue{(+2.7)}& &\blue{(+2.4)}& &\blue{(+1.4)}\cr\specialrule{.2em}{.1em}{.1em} \specialrule{.2em}{.1em}{.1em}
    CMPAE{$\dag$} \cite{gao2023collecting}& &{\bf64.2}&48.9 & 66.4&61.7& 59.2& 63.3&55.5&{\bf62.8}&37.6& & 56.6&43.8& 63.7&61.1& 51.8& 51.9&50.3& {\bf55.7}&34.0\cr \cmidrule{1-21}
    {{\method}}{$\dag$} & & {\bf 64.2}&{\bf49.6}& \bf{67.1}&{\bf63.1}& \bf{59.8}& \bf{63.8}&{\bf57.0}&{61.9}&{\bf38.4}& & {\bf57.1}&{\bf45.0}& {\bf64.8}&{\bf62.7}& {\bf52.8}&{\bf58.2}&{\bf52.4} & {55.5}&{\bf34.6}\cr 
    & & &\blue{(+0.7)}& &\blue{(+1.4)}& \blue{(+0.6)}& &\blue{(+1.5)}&~~&\blue{(+0.8)}& & &\blue{(+1.2)}& &\blue{(+1.6)}& \blue{(+1.0)}& &\blue{(+2.1)}& &\blue{(+0.6)}\cr\specialrule{.2em}{.1em}{.1em}
  \end{tabular}
  }
\end{table}

\begin{table}[t]
\centering
\scalebox{0.75}
{ \hspace{-7.3mm}
  \setlength{\tabcolsep}{0.1pt} % Default value: 6pt
    \renewcommand{\arraystretch}{1.0} % Default value: 1
  \begin{tabular}{@{}l c ccccccccc c ccccccccc @{}}\specialrule{.2em}{.1em}{.1em}
    \multirow{2}{*}{Method}&\phantom & \multicolumn{9}{c}{Segment-level (\%)}&\phantom & \multicolumn{9}{c}{Event-level (\%)}\\ \cmidrule{3-11} \cmidrule{13-21}
    & \phantom & A&Ao& V&Vo& AV& T@&T@o & E@&E@o&\phantom& A&Ao& V&Vo& AV& T@&T@o & E@&E@o\\ \specialrule{.2em}{.1em}{.1em}
    % HAN \cite{tian2020unified},ECCV2020 & & 61.1/& 62.9/& 57.2& 60.4/&59.5/& & 54.0/& 58.5/& 50.3& 54.3/& 51.2/\\
    % MA \cite{wu2021exploring},CVPR2021& & 61.3/&64.2/ & 57.6& 61.0/&59.8/& & 54.1/& 60.3/& 51.4& 55.3/& 51.9/\\
    JoMoLD \cite{cheng2022joint}& & 61.5&46.3& \underline{64.7}&64.8& 58.3& 61.5&56.5&60.3&38.0& & 54.7&41.5& 61.5&63.5& 52.4& 56.2&52.5&53.1&33.6\\
    % AVSDN \cite{?},arxiv2023 & & 60.5/& 64.8/& 58.3& 61.3/&59.4/& & 51.4/& 61.5/& 51.2& 54.7/& 50.8/\\
    CMPAE \cite{gao2023collecting}& & \underline{ 64.1}&48.5&64.3&\underline{66.9} & \underline{58.9}& \underline{62.4}&\underline{58.1}&\underline{62.0}&{40.0}& & \underline{57.0}&42.7& 62.1&\underline{66.0}& \underline{53.5}& \underline{57.6}&\underline{54.1}& 55.0&35.1\\ 
    VALOR \cite{lai2023modality} & & 61.8&\underline{49.0}& {\bf65.9}&66.7& 58.4&62.0&57.9 &61.5&\underline{40.8}& &55.4&\underline{44.2} &\underline{62.6}&65.0 &52.2 &56.7&53.8 & \underline{54.2}&\underline{35.8}\\\cmidrule{1-21}
    % {{\method}} (wo CLIP \& CLAP labels) & & {\bf{64.2}}/{49.3}& {64.7}/{60.3}& {58.1}& {62.3}/{55.8}&\underline{62.3}/{37.8}& & {\bf57.4}/{44.7}& {62.0}/{59.8}& {51.1}&{56.9}/{51.8} & {\bf55.8}/{34.1}\cr 
    {{\method}} & & \bf{64.2}&{\bf{51.2}}& {64.4}&{\bf67.7}& {\bf59.3}& {\bf62.6}&{\bf59.4}&{\bf62.5}&{\bf41.3}&~~& \bf{57.6}&{\bf45.5} &{\bf63.2}&{\bf67.0} & {\bf54.2}&{\bf57.9}&{\bf55.6} & \bf{55.6}&{\bf36.4}\cr
    & & &\blue{(+2.2)}& &\blue{(+0.8)}& \blue{(+0.4)}& &\blue{(+1.3)}&&\blue{(+0.5)}& & &\blue{(+1.3)}& &\blue{(+1.0)}& \blue{(+0.7)}& &\blue{(+1.5)}& &\blue{(+0.6)}\cr\specialrule{.2em}{.1em}{.1em} 
  \end{tabular}
  }
  \caption{Weakly supervised AVVP results on the LLP dataset when utilizing video-level labels and CLIP and CLAP annotations for training. All methods use VGGish, ResNet152, and R(2+1)D to generate the input tokens (see Table~\ref{tab: SOTA-weak} for more definitions and terms).\vspace{-3mm}}
  \label{tab: clip and clap}
\end{table}


Table~\ref{tab: SOTA-weak} presents comparative results on the LLP dataset when only video-level labels are used for training. Table~\ref{tab: SOTA-weak} demonstrates that our proposed approach {\method} achieves new state-of-the-art results on all new metrics, \fsn{as well as AV under both standard and `selected thresholds’ settings}. {\method} exhibits over {\bf 1.1\%} F-score improvement on most new metrics. Specifically, it significantly increases Vo and Event@Avo by {\bf 3.6\%} and {\bf 2.0\%} F-score at the segment level, and Vo, AV, and Type@Avo by {\bf 2.2\%}, {\bf 2.7\%}, and {\bf 2.4\%} F-score at the event level (under the standard setting), \fsn{and Type@Avo by {\bf 2.2\%} F-score at the event level (under the `selected thresholds’ setting).} On average across new metrics and AV, our proposed method improves the state-of-the-art results by 1.9\% and {1.2\% F-score} under standard and selected threshold settings, respectively. 

% Furthermore, comparing {\method}' performance with CMPAE, employed as {\a}'s backbone, demonstrates  1.7\% F-score improvement on average across new metrics and AV (standard setting), 



\vspace{1.0mm}
\noindent{\bf Analysis of Metrics --} In Section~\ref{sec: metrics}, we stated that the traditional A and V metrics do not adequately reflect the method’s ability to detect audible-only and visible-only events, respectively. As in the A and V metrics, apart from counting audible-only and visible-only events, respectively, they mistakenly include audible-visible events as true positive. This can have a detrimental impact on the analysis of the method's performance. For example, using the traditional A metric, HAN and MA \cite{wu2021exploring} appear to show nearly identical performance in detecting audible-only events at 60.1\% and 60.3\% F-score (at segment-level), respectively. However, when we evaluate them using our proposed Ao metric that counts correctly audible-only events, we observe that MA outperforms HAN with a margin of 10.4\%.  Similarly, based on the V metric (at event-level), CMPAE \cite{gao2023collecting} outperforms JoMoLD in detecting visible-only events, while our proposed Vo metric reveals that JoMoLD achieves a better performance than CMPAE. Consequently, the traditional Type@AV and Event@AV have similar issues.

\noindent{\bf Qualitative Results --} \fsn{In Fig.~\ref{fig:qualitative}, we qualitatively compare {\method} with the state-of-the-art CMPAE \cite{gao2023collecting} and JoMoLD \cite{cheng2022joint} on a test video sample of LLP. 
% Fig.~\ref{fig:qualitative} shows that for
For the `Singing' event, while CMPAE classifies it as audible-visible and JoMoLD does not recognize it, {\method} correctly recognizes it as audible-only. For the audible-visible event `Violin,' {\method}'s event predictions have a better overlap with the ground-truth annotations than the other approaches.}

\begin{figure}[t]
\CenterFloatBoxes
\begin{floatrow}
\ffigbox
  {\includegraphics[width=1.0\linewidth]{Figuers/qualitative.png}
  \caption{Qualitative comparison with previous AVVP approches (JoMoLD \cite{cheng2022joint} and CMPAE \cite{gao2023collecting}) using weak labels for training.}
  \label{fig:qualitative}}
\killfloatstyle
\ttabbox
{ \scalebox{0.9}
{
\begin{tabular}{@{}lcc @{}}\specialrule{.2em}{.1em}{.1em}
    {Method} & {AV (Seg)}& {AV (Evn)}\cr \specialrule{.2em}{.1em}{.1em}
     HAN \cite{tian2020unified}& 35.0& 41.4\cr
     MA \cite{wu2021exploring} & 37.9& \underline{44.8}\cr
     JoMoLD \cite{cheng2022joint} & 36.4& 41.2\cr
     CMPAE \cite{gao2023collecting} & \underline{39.7}& 43.8\cr \cmidrule{1-3}
     {\method}& {\bf41.5}~\blue{(+1.8)}& {\bf47.8}~\blue{(+3.0)}\cr\specialrule{.2em}{.1em}{.1em} 
  \end{tabular}
  }}
  {\caption{Weakly supervised AVE results on the UnAV-100 dataset. All methods use pre-trained VGGish \cite{hershey2017cnn} and two-stream I3D \cite{ carreira2017quo} to generate the input tokens. The best and the second-best results are in {\bf Bold} and \underline{underlined}, respectively.}
  \label{tab: AVE results}}
\end{floatrow}
\end{figure}

% The primary objective in Table \ref{tab: SOTA-weak} and our proposed approach is to address 
\noindent{\bf CLIP and CLAP Annotations --} Table~\ref{tab: SOTA-weak} addresses
the weakly supervised AVVP task without the need for additional annotations.
% Concurrent to ours, 
% Concurrent to ours,
The authors in \cite{lai2023modality} generate offline dense modality-specific annotations for the LLP dataset
% by utilizing 
with
large-scale pretrained models, CLIP \cite{radford2021learning}, and CLAP \cite{wu2023large}. In Table~\ref{tab: clip and clap}, we present comparative results with recent state-of-the-art approaches in which the networks are additionally trained on these annotations. The results of JoMoLD \cite{cheng2022joint} and CMPAE \cite{gao2023collecting} were obtained by adapting their available code. The results demonstrate that in this scenario with the modality-specific pseudo labels, {\method} still improves the state-of-the-art approaches consistently across all new metrics and AV F-score.

% \begin{table}[tb]
% \centering
% \scalebox{0.8}
% { 
%   \setlength{\tabcolsep}{4pt} % Default value: 6pt
%     \renewcommand{\arraystretch}{0.9} % Default value: 1
%   \begin{tabular}{@{}l ccc @{}}\specialrule{.2em}{.1em}{.1em}
%     {Method}&\phantom & {AV (Segment-level)}& {AV (Event-level)}\cr \specialrule{.2em}{.1em}{.1em}
%      HAN \cite{tian2020unified}, ECCV2020& & 35.0& 41.4\cr
%      MA \cite{wu2021exploring}, CVPR2021& & 37.9& \underline{44.8}\cr
%      JoMoLD \cite{cheng2022joint}, ECCV2022& & 36.4& 41.2\cr
%      CMPAE \cite{gao2023collecting}, CVPR2023& & \underline{39.7}& 43.8\cr \cmidrule{1-4}
%      {\method} & & ~~~~~~~~~~~{\bf41.5}~\blue{(+1.8)}& ~~~~~~~~~~~{\bf46.7}~\blue{(+1.9)}\cr\specialrule{.2em}{.1em}{.1em} 
    
%   \end{tabular}
%   }
%   \caption{Weakly supervised AVE results on the UnAV-100 dataset. All methods use pre-trained VGGish \cite{hershey2017cnn} and two-stream I3D \cite{ carreira2017quo} to generate the input tokens. The best and the second-best results are in {\bf Bold} and \underline{underlined}, respectively.}
%   \label{tab: AVE results}
% \end{table}

% \mbox{ }\vspace{1mm}
\subsection{{\method} for Audio-Visual Event Localization} 
To demonstrate the effectiveness of our proposed framework on another and a challenging dataset, we present the results of {\method} on the large-scale UnAV-100 dataset \cite{geng2023dense}. UnAV-100 has been captured for the Audio-Visual Event Localization (AVE) task, where the goal is to localize audible-visible events. UnAV-100 is the only existing AVE dataset in which the videos include multiple events, and the dataset covers 100 different action types, four times more than LLP. Unlike LLP with trimmed 10s videos, in UnAV-100, the videos are untrimmed, ranging from 0.2s to 60s. To obtain the weakly supervised results, for training, we derived the video-level labels from the videos' temporal annotations (see supp. file for the implementation details for this task). The results of other state-of-the-art approaches were provided through their available code. Comparative results on UnAV-100 using AV F-score are available in Table \ref{tab: AVE results}. It is shown that {\method} outperforms the other approaches by {\bf 1.8\%} and {\bf 3.0\%} AV F-score at the segment and event levels, respectively, and achieves state-of-the-art results on this dataset. 

% \begin{table}[!htb] 
% \scalebox{0.8}{
%   \floatsetup{captionskip=4pt}
%   \begin{floatrow}[2]
%   \hspace{-15mm}
%     \ttabbox%
%     {\begin{tabularx}{0.6\textwidth}{cccccccccc}
%       \toprule
%       method & A & V & AV & oA & oV & OAV & vv& bbbbbbbbb\\
%       \cmidrule(lr){2-2}\cmidrule(lr){3-3}
%       % $$ & 53.492 & 77.906 \\
%       % \addlinespace
%       % $$ & 46.753 & 61.587\\
%       \bottomrule
%       \end{tabularx}}
%     {\caption[Valori medi]{valori medi}
%       \label{tab:valaa}}
%     \hfill%
%     \ttabbox%
%     {\begin{tabularx}{0.6\textwidth}{c*{2}{>{\centering\arraybackslash}X}}
%       \toprule
%       & Sensibilità [$\%$] & Specificità [$\%$]\\
%       \cmidrule(lr){2-2}\cmidrule(lr){3-3}
%       $$ & 60\hphantom{.000} & 80.487 \\
%       \addlinespace
%       $$ & 54.545 & 67.777\\
%       \bottomrule
%       \end{tabularx}}
%     {\caption[Valori medi]{valori medi}
%  \label{tab:vala}}
%   \end{floatrow}
%   }
% \end{table}%   
